Video Analytics in Elite Soccer: A Distributed Computing Perspective

Ubiquitous sensors and Internet of Things (IoT) technologies have revolutionized the sports industry, providing new methodologies for planning, effective coordination of training, and match analysis post game. New methods, including machine learning, image and video processing, have been developed for performance evaluation, allowing the analyst to track the performance of a player in real-time. Following FIFA's 2015 approval of electronics performance and tracking system during games, performance data of a single player or the entire team is allowed to be collected using GPS-based wearables. Data from practice sessions outside the sporting arena is being collected in greater numbers than ever before. Realizing the significance of data in professional soccer, this paper presents video analytics, examines recent state-of-the-art literature in elite soccer, and summarizes existing real-time video analytics algorithms. We also discuss real-time crowdsourcing of the obtained data, tactical and technical performance, distributed computing and its importance in video analytics and propose a future research perspective.

==> takeout.tex <==
%Crowdsourcing technology has scaled up the fan\textquotesingle s engagement beyond 90 minutes of the match. The newly formed demands have pressured the sports clubs to innovate for surviving in this digital period. Fan\textquotesingle s not only seen to watch the live game but also they consume and share the contents in social media. Nowadays every clubs generate digital materials to get more share, tweets, and likes which helps them to convey the message and brings the fan closer providing them with the opportunity to engage in the game. The clubs utilize crowdsourcing technology by broadcasting specific task and asking fan\textquotesingle s to contribute with their feedback. These feedbacks are used to solve particular problems. With the strategy, they reinforce the fan\textquotesingle s experience which helps them to build trust among audiences and clubs. The clubs also benefit from the solutions that are a feasible, cost-effective and most importantly desired solution by their fan\textquotesingle s. Wearable technologies and has offered the new business model and have engaged more fan\textquotesingle s with the sophisticated and advanced products and applications.  However, most of the sports analytics tool available gives the summary after the game. 

%The structure of the paper is organized as follows: We present related work in section \ref{sec:literature_review}. We present in section \ref{sec:Background} the background on the field. In section \ref{sec:Individual Subjective Reports (PMSYS)} we discuss about Individual subjective reporting (PMSYS). We present in section Fog computing for the big data generated from the sport analytics in section \ref{sec:Fog_Computing_for_the_Big_Data_generated_from_ the_ Sport_ Analytics}. Section \ref{sec:Discussion} shows the sports specific based results; how resulting data are useful in consumer application and real-time crowdsourcing also briefly and discuss the overall work. Finally, we conclude our work in section \ref{sec:Conclusion and Future perspective}.

%Kim Hartvedt Andreassen et al. \cite{andreassen2018metrix} presented a thesis on Metrix, which is a digital toolkit for trainers to monitor their players throughout the practice or match. The system performs real-time analysis on recorded sensor data and is used for measuring the specific moment pattern of the players throughout the matches. Metrics provide trainers with a toolkit to individualize training burden to different playing positions on the field, or even to the participants itself. Ivan Baptista et al. \cite{baptista2018position} utilized time-motion analysis and triaxial-accelerometers to acquire new insights concerning the gaps in physical profiles of elite football players around the playing position. The positional differences in work pattern may assist coaches in developing individualized training programs to meet the requirements of each and every position in match-play. Besides providing invaluable information to coaches concerning the activity profiles, the results can also inspire a real-time personalization computerized coach toolkit which integrates with positional data in real-time. Svein A. Pettersen et al. \cite{pettersen2018quantified} share their experience of employing a detailed radio-based wearable positioning data approach in their elite soccer club. They demonstrated how much an entire system could find anomalies, trends, and understanding necessary for the individual athletes as well as for whole soccer team performance development. They discussed and compared the accuracy between radio waves and GPS in sampling monitoring data. They also presented the way they are appropriating for the extension of the radio-positional system with a novel soccer analytics system along with a real-time video processing method employing a video camera array. They expect the presented system could offer a new toolkit for contemporary forward-looking coaches. 



%The investigation for motion analysis started back at the 1970’s \cite{reilly1976motion}, where the coaches used pencil and paper (i.e., notational analysis) to record the field events. This involved observers on the sideline are recording the players' action on the field. Not only does this demands for a lot of time but also requires significant human resources. The notational analysis or manual investigation technique has certain limitations such as it fails to provide data regarding the speed or velocity metrics. Modern analysis technologies today consist of semi-automatic numerous camera-based systems, for instance, ProZone® along with Amisco Pro®, and athlete monitoring systems employing Global Positioning System (GPS), accelerometers, gyroscopes, and magnetometers (For instance, Catapultsports, STATSport, etc.).  The development of match and motion analysis has found data initially gathered using pen and pencil-based systems advancement to completely automatic computer-based system with the potential of documenting moves at the rate of 100 times a second to measure players moves in competition and training domain. These noteworthy advancements in the technology have significantly improved the efficiency, accuracy, and trustworthiness of the gathered data concerning to measurement of players locomotion. On the other hand, the usage of these different methodologies like semi-automatic various camera-based approaches and GPS based athlete monitoring devices for match evaluation inside the literature makes comparison difficult to explain without any standard method to estimate validity and reliability in competition environments \cite{coutts2010validity,cummins2013global,jennings2010variability}.

%Advancement to the traditional notation analysis is video-based time-motion analysis, requiring players to be filmed throughout the training or match \cite{bangsbo1991activity}. The footage is analyzed post-game, permitting the audience to pause, review and slow down the video motion to have the much closer look. We typically distinguish between two types of video analysis, namely collective and individual. With individual records, one camera follows one player. Its disadvantage is the need for a camera operator, in addition to missing contextual data with respect to the team altogether. The collective strategy simplifies this by utilizing one or even many cameras providing a summary of the field, able to record the videos of each of the players simultaneously. The disadvantage with this is the problem of quantifying individual players movement pattern accurately. 

%Together with all the current advancement of electronic technology, more semi-automated systems have altered the manual process of collecting individual player \textquotesingle s information. Probably, the most likely system is ProZone, (currently known as STATS), who at the early 2000s introduced a semi-automated video tracking approach employing many cameras put into pre-determined places at the stadium, within the whole field. During video image analysis, the player trajectory is set through coordinates X, and coordinate Y, which is calculated in meters from the center circle on the pitch, whose sampling rate is 10 Hz \cite{valter2006validation}. This enables calculation of space covered and average speed between the samples, effortlessly measuring players speed or velocity, and distance metrics. The semi-automated video tracking approach is still a popular approach for evaluating movement patterns of the players.

%Nevertheless, these approaches are restricted by their requirements of an observer for cleanup, structuring, and affirming the accumulated data, that \textquotesingle s a time-consuming procedure. Consumers of such investigation must usually expect a 24-hour wait until it’s readily available for them. Another drawback is the absence of portable system component, restricting match investigation to special training facilities which employs the static camera setup. The other frequent way of quantifying player movement pattern would be using the radio-based detector system \cite{wang2015review}. Here, each player wears a data processor which has the sensors throughout the physical activity. The sensor sends signals to wireless recipients, typically installed on antennas located around the perimeter of the pitch. The radio frequency based technology helps observer to track players with high accuracy. 

%Some systems also encourage integration using supplement equipment, for instance, heart-rate tracker or accelerometers, offering additional data of players performance metrics. The very renown system to hire a radio-based system approach is ZXY sports Tracking \cite{CHYRONHEGO}, which we will discuss later. Very similar to this semi-automated system, many radio-based systems have been set up as stationary installations, which restricts their usage to special training facilities. Throughout its drawbacks include sophistication of setup, radio-based systems are thought to be non-invasive and accurate for all those players. 

%Through remarkable advances in engineering, the growth of motion analysis has evolved from data initially accumulated with paper and pencil into completely automatic computer technologies capable of shooting fine motion patterns on the area. These advancements have significantly increased efficacy, accuracy, and reliability of measuring soccer players throughout practice or match. Recently many commercialized products, such as GPS units are available for sports tracking. These devices have become increasingly more popular for measuring the performance metrics of the player \cite{wisbey2010quantifying}. System utilizing this technology comprises of ZXY sports Tracking \cite{CHYRONHEGO}, GPSports \cite{D}, CatapultSports \cite{E} and also StatSports \cite{Statsports}. Together with advancements in GPS technology, the components of the sensor have decreased significantly concerning their size. They are non-invasive. Thus, players can wear them underneath their clothing during the game or practice.

%With high-frequency sampling rates, sensor units record physical performance parameter with huge accuracy, providing information like speed, acceleration, and distance covered, in addition to positional data to track the player during a match on the field. Opposite into semi-automated solutions, GPS components are mobile, letting them be used at either home and away games. Sensor data is automatically recorded and stored, permitting automatic analysis applications to additional process its material through data aggregation and filtering. Through noteworthy technological advancement, the growth of motion analysis has evolved from data initially accumulated with paper and pencil to an utterly automatic computer system that is capable of recording even tiny movement during the match. These advancements have significantly increased efficacy, accuracy, and reliability of quantifying soccer players during the game.


%Football has definitely become an open-loop game, so it becomes crucial to highlight the requirement for further research to a legitimate indication of our own comprehension of the valid sign of physical match performance and competitive victory ~\cite{carling2013interpreting}. The athletic quantification technologies already set up in the research at Alfheim Stadium has already been generating essential insight. At Alfheim Stadium, there has become a significant emergence and use of numerous tracking or monitoring technology. They include GPS and LPM systems which are introduced briefly above. Each of these tracking technologies is capable of speedy recording and saving data of the team players. We must move from GPS-based technological innovation, that’s become more preferred choice from the clubs for quantifying training load of team sports athletics player, both throughout the game and training ~\cite{aughey2010australian}. A different to GPS based methods are those who are dependent on LPM radio signals. [42 ChyronHego et al. (Trondheim, Norway] has many years of experience in working with the positional tracking utilizing stationary LPM system, i.e., ZXY Sport Tracking System.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics{LPM.jpg}
%     \caption{LPM System ~\cite{J}}
%     \label{fig:my_label}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.8]{Receiver-antenna-for-the-ZXY-system.png}
%     \caption{Receiver antenna for the XZY system placed at Alfheim stadium}
%     \label{fig:my_label}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{image.jpeg}
%     \caption{Oveall Bagdus architecture ~\cite{stensland2014bagadus}}
%     \label{fig:my_label}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5



%The cameras have been mounted in a circular layout, each covering a distinct portion of the soccer field, as exhibited in Figure 4. 

%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{stiching.eps}
%     \caption{Camera setup at the stadium ~\cite{gaddam2018camera}}
%     \label{fig:my_label}
% \end{figure}
%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.4]{cameraframe.eps}
%     \caption{Panorama examples from Alfheim stadium and Ullevaal stadium ~\cite{gaddam2018camera}}
%     \label{fig:my_label}
% \end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{Fog_computingg.png}
%     \caption{Different interaction models in fog computing ~\cite{simmhan2017big}}
%     \label{fig:my_label}
% \end{figure}

%Gaddam et al. implemented similar ideas in a real-time interactive panoramic video system. They showed that their algorithm that progressively increases in quality toward the standpoint find a way to reduce the bandwidth demand and offer a similar quality of experience (QoE) as a full panorama system.

%Michelsen et al.~\cite{michelsen2015herakles} demonstrated a system for live sports analysis employing streaming sensor data and a Peer-to-Peer network of regular and low-cost privately-owned machines. Zhang~\cite{zhang2014controlled} presented a code consent, which is a user-centric device that attaches informed consent and capabilities to allow athletes to distribute their private information more controllable way. 

%Also, the driving force for this improvement is development in the sensor technology and the coverage of the sports in the media channel. Previously, performance analysis mainly depended on a frequency distribution of sports organized.
%In contrast, the current novel techniques allow in calculating more intricate metrics that are helpful to quantify the performance of individual players and the whole team. 
%Therefore, many sports industries are adopting computer-aided sports analytical approaches for making decisions since analytics has been proven to contribute to success. 

%The algorithmic evaluation from the collected data may be useful during training, substitutions, designing physical workout sessions, evaluating fitness levels, planning strategies, monitoring fatigue, and injury prevention. 


% The technical or practical components of match analysis include the quality of skills implemented by players at a match. The tactical component identifies the plan, strategy, and style of the game, whereas the physical component includes quantified movement patterns and overall efforts made by players on the ground. Therefore, a match analysis might focus on various aspects of the game, from the specific individual on the ground to a composite investigation of the interplay between each of the team's players around the ball \textemdash processing method employing a video camera array. They expect the presented system could offer a new toolkit for contemporary forward-looking coaches. 



% The IoT systems, for example, wearable sensors, tablet, and mobile phones generate an enormous amount of data but usually have inadequate resources to process these generated data at the edge. The IoT-based technologies are currently employed only in the leading domestic competitions and at major international games for financial purposes~\cite{toka2017resource}. The reason for this is, at present, there is severe engineering difficulty to build such systems at an affordable cost. The principal cause of the high cost is the dedicated hardware that controls the time-critical processing of a large volume of data on-site. Cloud computing would give a cost-efficient solution, and we can predict that shortly, the IoT-based technologies will find their way into leisure sports to facilitate through low-cost cameras and sensors around the ground, supported by service-oriented cloud-based data analytics. However, for a cloud-based system, we must consider two constraints. They are low latency for real-time utilization of specific applications and affordable uplink speed. Many time-critical IoT situations have developed and created hurdles while promoting low latency applications. Simultaneously, cloud computing successfully delivered computing as a service at a budget price with excellent scalability and high security. Therefore, IoT devices are seen hugely benefiting from a cloud-based backend. 

%However, while researchers have made considerable advancements, there are significant hurdles that need to be addressed. 

%Their prototypes were developed at Alfheim Stadium (Tromsø IL, Norway), and they utilized a dataset captured at a Norwegian premier league game to signify their system. Gaddam et al.~\cite{gaddam2016tiling} applied tiling to deliver different quality levels for various parts of the panorama. Tilling has been used for delivering high-resolution content to customers.


% For instance, GPS, Player tracking technology offers descriptive information in quantifying movement patterns and physical status in training.

% The system traces the individual by zooming in, playback events from the matches with stitched panorama video, and making video summaries based on questions to the sensor system.

%Digital technology has an impact on every industry, every service, and every corner of the increasingly connected world~\cite{attaran2021impact}. Advancements in digital technology are changing the sports industry as well~\cite{ratten2019sport}. For instance, sports coverage, buying tickets, and designing equipment (shoes) are much more efficient. Live streaming, virtual reality, over-the-top service delivery, mobile applications, performance insights, and real-time highlights make a digital landscape that has influenced the worldwide sports industry. 


The product of the company especially targets the soccer community providing a range of commodities, such as tracking balls and players on the ground, tracking the physical performance of the players, wearable belts, transponders, and collecting those statistical data from compressed belts and tight shirts with a transponder for the post-session analytics. 


You mainly talk about VIDEO analytics - there are much other work in context pdf analytics to like subjective reports, player tracking using GPS, etc.




%  \subsection{Video system}
% The video system is made of multiple small shutter vulnerability synchronized cameras that capture high-resolution video of the soccer ground. The cameras have been set up to cover the full field complete area with sufficient heed to recognize common attributes required for the camera calibration and stitching of the panorama frame. 


% \subsubsection{Camera setup}
% In order to cover the entire field, Bagadus utilize five 2K Basler industry vision camera ~\cite{gaddam2018camera}. Each camera provides a maximum resolution of 2046 $\times$ 1086 pixel. The frame rate per second (fps) is 50 over Gigabit Ethernet. To optimize the panorama resolution, the cameras have been rotated by 90 degrees, providing a per-camera field of view of 66 degrees~\cite{gaddam2018camera}.


%\subsubsection{Video Processing Pipeline}
%The camera output signal is processed by way of a custom real-time video pipeline~\cite{stensland2014processing,tennoe2013efficient} to boost the live video feeds. Most of the pipeline components can use both the Graphical Processing Unit (GPU) and Central Processing Unit (CPU) and~\cite{wilhelmsen2014using,stensland2015using} processing of the data with higher performance. %Figure 5 exemplifies the data processing utilized at the Bagadus deployments, using samples of individual captured video frames as shown in Figure 5a. Figure 5b demonstrates how these captured frames are stitched together at overlapping regions by a vigorously calculated seam. Figure 5c shows the final panorama video that has a frame resolution of 4096 $\times$ 1680 pixels and is encoded and compacted together with the x264 encoder ~\cite{aimarvideolan} Advanced Video Coding (AVC) compression format. Figure 5d shows the ulleval stadium, and it can be seen from the figure that the visual output is perfect. 

%Along with the smartphone app, they also constructed a web portal that team coaches utilize to summarize and present data. Coaches can access the portal with several tools and valuable plots for each player and team. Also, with the web portal and software (mobile applications), they have implemented their communication services between the cellular phone and their web portal, allowing their trainer to send 1PMSys, push-messages precisely to an individual player's cellular phone. 

%A vital property of PMSys is the intelligence for coaches to plan the future and replicate the push messages. The team 's experiences with PMSys Athlete Self-Report Measures (ASRM) at Alfheim is that education and feedback are most important for maintaining the daily usages. The education scopes at including why an ASRM should be utilized, the intention behind the query, and who is accessing and summarizing the data. Education should highlight that the outcomes are utilized for the benefit of players, and feedback should contain the daily interactions and reminders revealing exactly what actions are required in reaction to the data accessed from the players. The reports generated daily can be the baseline for regular discussion between coaches and players. The involvement of the staff, mainly during the implementation process, is vital ~\cite{halvorsen2013bagadus} for responding day to day response to the staff and analyzing and interpreting the ASRM. This system would be of great importance as it could help predict the injury and the performance of the individual players. Even additional inputs could be beneficial for machine learning models for making the prediction. 


%In the context of computer systems, to deal with the technical challenges, numerous issues need to be addressed to provide real-time operations. In this respect, the Bagadus soccer analysis application integrates a sensor system, soccer analytics annotations and video processing of a video camera array. There are some problems with Bagadus, like camera calibration problems, parallax errors, managing the variations in the lighting conditions, etc. There are more problems related to suboptimal auto exposure, time synchronization at several levels, and insufficient dynamic range on the camera sensors. Although the GPU implementation has already been tested, there is a high potential on the GPU for scaling the pipeline to have a higher resolution with more cameras. 


%The conventional approach has been used for four years to measure the physical performances of the match. On the other hand, the integrated strategy contextualizes by assimilating physical and strategic or tactical data efficiently. 


%Fog computing decreases the distance that data must travel over the network. As a consequence, the latency and bandwidth costs are reduced, and one can derive quick insights for making more timely decisions in real-time. 



%Bagadus, a real-time system for sports analysis, provided automatic processing and retrieval of all the events from the sports stadium.
%The image quality of the video can be further improved by using high-resolution camera and processing speed can be improved employing GPUs. 

